When Is Inductive Inference Possible?

Can a physicist make only a finite number of errors in the eternal quest to uncover the law of nature? This millennium-old philosophical problem, known as inductive inference, lies at the heart of epistemology. Despite its significance to understanding human reasoning, a rigorous justification of inductive inference has remained elusive. At a high level, inductive inference asks whether one can make at most finite errors amidst an infinite sequence of observations, when deducing the correct hypothesis from a given hypothesis class. Historically, the only theoretical guarantee has been that if the hypothesis class is countable, inductive inference is possible, as exemplified by Solomonoff induction for learning Turing machines. In this paper, we provide a tight characterization of inductive inference by establishing a novel link to online learning theory. As our main result, we prove that inductive inference is possible if and only if the hypothesis class is a countable union of online learnable classes, potentially with an uncountable size, no matter the observations are adaptively chosen or iid sampled. Moreover, the same condition is also sufficient and necessary in the agnostic setting, where any hypothesis class meeting this criterion enjoys an $\tilde{O}(\sqrt{T})$ regret bound for any time step $T$, while others require an arbitrarily slow rate of regret. Our main technical tool is a novel non-uniform online learning framework, which may be of independent interest.

==> backup.tex <==
\begin{definition}[Finite-error cover]
Given any hypothesis class $\mathcal{H}$, we say $h$ is a finite-error cover of $\mathcal{H}$, if 
$$
\forall h'\in \mathcal{H}, |h(x)\ne h'(x)|<\infty.
$$
Furthermore, we say $\mathcal{H}$ has a countable finite-error cover, if there exists countable number of sets $\mathcal{H}_n$ and $h'_n\in \mathcal{H}_n$, such that
$$
\mathcal{H}=\cup_{n\in \mathbb{N}^+} \mathcal{H}_n, h'_n\ \text{is a finite-error cover of}\ \mathcal{H}_n.
$$    
\end{definition}
We have the following result which characterizes strongly-EAS learnability:
\begin{theorem}
    $\mathcal{H}$ is strongly-EAS-learnable if and only if $\mathcal{H}$ has a countable finite-error cover.
\end{theorem}
\begin{proof}
We discuss the two directions respectively. The proof is similar to \cite{wu2021non} in spirit.

\textbf{Only if:} Suppose $\mathcal{H}$ has a countable finite-error cover $\mathcal{H}_n$ with $h'_n$ as above. We describe an algorithm $\mathcal{A}_n$ which strongly-EAS learns $\mathcal{H}_n$. 

The algorithm maintains a set $W_n$ of points which it made mistakes on in the past, initially set as $\emptyset$. At time $t$, the algorithms checks if $x_t\in W_n$. If yes, it predicts the correct label which it has seen. Otherwise it predicts $h'_n(x_t)$, then adds $x_t$ to $W_n$ if the prediction is wrong. Clearly, the algorithm makes at most $|h^*(x)\ne h'_n(x)|$ mistakes when $h^*$ is the ground-truth hypothesis.

Now, we describe an algorithm $\mathcal{A}$ for strongly-EAS learns $\mathcal{H}$. Denote $e(t,n)$ as the the number of errors that $\mathcal{A}_n$ would made if it were employed in the first $t-1$ steps, let
$$
J_t=\argmin_{n}\{e(t,n)+n\},
$$
the algorithm $\mathcal{A}$ predicts as $\mathcal{A}_{J_t}$ at time $t$.

Assume the ground-truth hypothesis $h^*$ lies in $\mathcal{H}_k$, then $\mathcal{A}_k$ makes $|h^*(x)\ne h'_k(x)|$ errors which is finite, denoted as $s$ for simplicity. We have that $e(t,k)+k\le s+k$ for any $t$. Therefore, we have that $J_t\le s+k$ for any $t$, meaning $\mathcal{H}$ only invokes $\mathcal{A}_1,\cdots,\mathcal{A}_{s+k}$. Furthermore, once an $\mathcal{A}_n$ makes more than $s+k$ errors, it will not be chosen by $\mathcal{A}$ anymore, thus $\mathcal{A}$ makes at most $(s+k)^2$ errors, which is finite.

\textbf{If:} Suppose $\mathcal{H}$ is strongly-EAS learnable. We may assume without loss of generality such that $\forall h_1,h_2\in \mathcal{H}, |h_1(x)\ne h_2(x)|\ge \aleph_0$.  Note that any hypothesis class can be reduced to one, denoted as $\hat{\mathcal{H}}$, satisfying the above property by choosing a representative function in each equivalence class defined by the relation $h_1\sim h_2: |h_1(x)\ne h_2(x)|<\infty$. Then $\hat{\mathcal{H}}$ is also strongly-EAS learnable, by invoking the algorithm which strongly-EAS learns $\mathcal{H}$.

Now, we prove that if $\mathcal{H}$ is strongly-EAS-learnable, then $|\mathcal{H}|\le \aleph_0$. Equivalently, this is to say if $\mathcal{H}$ admits a function $\mathcal{A}: (\mathcal{X}\times\{0,1\})^*\times\mathcal{X}\to \{0,1\}$ such that $\forall h\in \mathcal{H}$ and $\forall \mu$,
$$
\mathbb{P}\left(\sum_{t=1}^{\infty} 1\{\mathcal{A}(Z_{t-1},x_t)\ne h(x_t) \}<\infty \right)=1,
$$
where $Z_{t-1}=(z_1,\cdots,z_{t-1})$ and $z_t=(x_t,h(x_t))$, then $\mathcal{H}$ is countable.

\zl{so far}

Define the event
$$
A_n^h=\left\{x: \sum_{t=n}^{\infty} 1\{\mathcal{A}(Z_t,x_{t+1})\ne h(x_{t+1}) \}>0\right\},
$$
and define the hypothesis class 
$$
\mathcal{H}_n=\left\{h\in \mathcal{H}: \forall \mu, \mathbb{P}(A_n^h)\le \frac{1}{4}  \right\}.
$$
By the definition of $\mathcal{H}_n$, we have that $\mathcal{H}=\cup_{n\in \mathbb{N}^+}\mathcal{H}_n$, because for any $h$ and $\mu$ we have $\lim_{n\to \infty} \mathbb{P}(A_n^h)=0$ by the strongly-EAS learnability. As a result, we only need to show each $\mathcal{H}_n$ is countable.

We claim that for any $\mathcal{H}_n$,
$$
\sup_{\mu} \inf_{h_1\ne h_2\in \mathcal{H}_n} \{\mathbb{P}_{x\sim \mu}(h_1(x)\ne h_2(x))\}>0.
$$
This will imply $\mathcal{H}_n$ is countable, because

\zl{bad example: translation of all reals in $[0,1]$}

\end{proof}

\section{Characterizing Adaptive-EAS Learnability}
\begin{theorem}
    $\mathcal{H}$ is adaptive-EAS learnable if and only if $\mathcal{H}$ is pointwise-adaptive-EAS learnable.
\end{theorem}
\begin{proof}
By the inclusion relation, we only need to discuss the only if direction. It's equivalent to show that (1) $\mathcal{H}$ is adaptive-EAS learnable, and (2) $\mathcal{H}$ is not pointwise-adaptive-EAS learnable, are incompatible.

To this end, we will first regularize the behaviours of the learner and Nature to avoid some ill situations. We can assume without loss of generality that $y_t=h(x_i)$ whenever there exists $x_i=x_t,i<t$, since it never increases the number of errors made for any given $h,x$. Conditioned on this, we can assume $x_i\ne x_j, \forall i\ne j$ for Nature. We can also obtain a new algorithm $\mathcal{A}'$ by setting $$
y'_t|\cup_{i<t}(x_i,h(x_i)) \cup \{x_t\}=y_t|\cup_{i<t,h(x_i)\ne y_i}(x_i,h(x_i)) \cup \{x_t\}.
$$
For any $h$, $\mathcal{A}'$ also makes finite errors. In addition, there is a uniform error bound on $h$ for $\mathcal{A}'$ if and only if there is a uniform error bound on $h$ for $\mathcal{A}$. 

Finally, we can assume $y_t: \cup_{i<t}(x_i,h(x_i)) \cup \{x_t\}\to \{0,1\}$, that the current prediction doesn't depend on the order of history samples. For the same reason as above, it preserves both (non) learnabilities. Conditioned on all above, we can restrict our consideration to $x$ such that $|h(x_i)-y_i|\ge |h(x_j)-y_j|, \forall i<j$, noticing that $x$ can depend on $\mathcal{A}$.

Now, suppose (1) and (2) hold at the same time, we would like to derive a contradiction. By (1) and (2), there exists an algorithm $\mathcal{A}$ of learner and a $h \in\mathcal{H}$, such that for any Nature's choice of $x$ we have $A(x)<\infty$, but for any $n$ there exists $x$ that $A(x)\ge n$,where $A(x)$ denotes the number of errors made by $\mathcal{A}$ on $h$. We fix this $h$ and focus on $x$ afterwards.

We define $X_n=\{x: A(x)\ge n\}$. Clearly, every $X_n$ is non-empty. Moreover, every $X_n$ is infinite, otherwise $\mathcal{A}$ makes at most $n+|X_n|$ errors. Now, we want to construct $x_1,\cdots$ such that $\mathcal{A}$ makes an error on every $x_t$. 

We first find $x_1\in X_1$, such that 

\zl{tbd}

\zl{very bad example}

\zl{On countable domain, pointwise=EAS!!!}

(2) means for any algorithm $\mathcal{A}$, there exists $h$, such that for any $n$, there is $x$ that $err(h,x)\ge n$.

(1) is equal to countable tree of $(h,x)$ pair?

If (1) (2) holds, then there are uncountable $h$ which are not pointwise.

there is $x$ with uncountable $h(x)$ is a sufficient condition for not (1).

Consider a shatter tree, both threshold and finite support has countable $h(x)$ and uncountable $h$ on every $x$. what's the key difference?

\end{proof}

\section{Special Cases}

When $\mathcal{X}$ is countable, PAEAS=EAS.

When $\mathcal{X}=[0,1]$ and $\mathcal{H}$ is measurable?

\section{Characterizing Strongly-EAS Learnability}
\begin{theorem}
    $\mathcal{H}$ is strongly-EAS learnable if and only if $\mathcal{H}$ is adaptive-EAS learnable.
\end{theorem}
\begin{proof}
By the inclusion relation, we only need to discuss the only if direction. It's equivalent to show that (1) $\mathcal{H}$ is strongly-EAS learnable, and (2) $\mathcal{H}$ is not adaptive-EAS learnable, are incompatible. We begin with the following definition.

\begin{definition}[Duplicate-permutation extension]
    For any countable set $\cup_{i\in \mathbb{N}^+} \{x_i\}$ (without loss of generality we require $x_i\ne x_j, \forall i\ne j$), we say an ordered countable sequence $\Pi_{i\in \mathbb{N}^+}\{z_i\}$ is a duplicate-permutation extension of $\cup_{i\in \mathbb{N}^+} \{x_i\}$, if for any $j\in \mathbb{N}^+$ we have $ z_j\in \cup_{i\in \mathbb{N}^+} \{x_i\}$ and $ x_j\in \cup_{i\in \mathbb{N}^+} \{z_i\}$. We denote the set of all such duplicate-permutation extensions as $DPE(\cup_{i\in \mathbb{N}^+} \{x_i\})$.
\end{definition}

We first prove a claim that when (2) holds, for any $\mathcal{A}$, there exists $h$ and $X=\cup_{i\in \mathbb{N}^+} \{x_i\}$ such that $\mathcal{A}$ makes infinite mistakes on every sequence $x\in DPE(X)$. 

Otherwise, there exists an algorithm $\mathcal{A}$, such that for any pair of $h$ and $X=\cup_{i\in \mathbb{N}^+} \{x_i\}$, there is a sequence $x^* \in DPE(X)$ that $\mathcal{A}$ makes finite errors on.

We will show that, based on this $\mathcal{A}$, we can prove the existence of a new algorithm $\mathcal{A}^*$ such that it makes finite errors on any $x\in \mathcal{X}^{\aleph_0}$, which will contradicts (2) and thereby prove the claim.

We first modify $\mathcal{A}$ such that it predicts $y_t=h(x_t)$ whenever there exists $i<t$ such that $x_i=x_t$ meaning the true label $h(x_t)=h(x_i)$ is already known to Learner, and predicts as if the original $\mathcal{A}$ was adopted for other $x_t$. Notice such modification won't increase the number of errors made for any $h,x$.

Now, fix any pair of $h$ and $X$, and denote $T$ as the first time step such that $\mathcal{A}$ makes no error on $x^*_t$ for any $t>T$, which is finite. For any other $x'\in DEP(X)$, denote $T'$ as the first time step that $\cup_{i=1}^T\{ x^*_i\}\subset \cup_{i=1}^{T'}\{ x^{'}_i\}$, which is also finite. For any $t>T'$ satisfying $x_t\ne x_i$ for all $i\le T'$, denote $t'$ as the first time step such that $x^*_{t'}=x^{'}_t$ which is finite, the new algorithm $\mathcal{A}^*$ confidently predicts $y_t=h(x^*_{t'})$, by 'consulting' $\mathcal{A}$ with $T'$ serving as a certificate. 

We also need to show for two different $h_1,h_2$, the certificates are also different. \zl{check}

As a result, the new algorithm makes at most $t$ errors for any $h$ and any sequence $x$ with countable size of $\cup_{i\in \mathbb{N}^+} \{x_i\}$. For any sequence $x$ with finite size of $\cup_{i\in \mathbb{N}^+} \{x_i\}$, by the first modification, it makes at most $|\cup_{i\in \mathbb{N}^+} \{x_i\}|$ errors. We conclude the proof of the claim.

Now that the claim is proved, let $\mathcal{A}$ be an algorithm satisfying (1), and $h$ and $X=\cup_{i\in \mathbb{N}^+} \{x_i\}$ such that $\mathcal{A}$ makes infinite mistakes on every sequence $x\in DPE(X)$. We fix any full-support discrete probability measure $\mu$ on $X$, for example, the measure induced by $\mu(x_i)=\frac{1}{2^i}$. Under iid generation of samples under $\mu$, with probability 1, we have that $x\in DPE(X)$, thus $\mathcal{A}$ makes infinite errors with probability 1 for $h$ and $\mu$, contradicting (1).

\end{proof}

\section{Determining Inclusion Relations}
We will start with determining the inclusion relations from easier to harder. 

\subsection{Online $\ne$ Adaptive-EAS}
Consider the learning problem with $\mathcal{X}=[0,1]$ and $\mathcal{H}=\{h: h(x)=1_{[x\ge q]}, q\in \mathbb{Q}\}$. This problem is clearly not online learnable, by letting Nature choose $x_t\in (\max_{i<t, x_i=0} x_i, \min_{i<t, x_i=1} x_i)$. On the other hand, this problem is adaptive-EAS learnable, \zl{tbd}

\subsection{Adaptive-EAS $\ne$ Strongly-EAS}

\subsection{EAS $\ne$ Strongly-EAS}
Consider $\mathcal{X}=[0,1]$ with the regular Borel $\sigma$-algebra $\mathcal{F}$. Let 
$$\mathcal{H}=\{h:|h^{-1}(1)|<\infty\}\cup \{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|<\infty, a_i,b_i\in \mathbb{Q}\}.$$
We have the following result which answers an open problem of \cite{wu2021non}:
\begin{theorem}
    $\mathcal{H}$ is EAS-learnable for any probability measure $\mu$, but not strongly-EAS-learnable.
\end{theorem}

\begin{proof}

Let $\lambda$ denote the Lebesgue measure over $[0,1]$. By the Lebesgue decomposition theorem on $\mathbb{R}$ \cite{hewitt2013real}, any regular Borel probability measure $\mu$ can be uniquely written as the sum of three $\sigma$-finite measures $\mu_1+\mu_2+\mu_3$ such that $\mu_1$ is absolutely continuous and dominated by $\lambda$, $\mu_2$ is continuous and singular to $\lambda$ and $\mu_3$ is discrete (supported on a at most countable set):
$$
\mu=\mu_1+\mu_2+\mu_3, \mu_1\ll \lambda, \mu_2 \perp \lambda, |\mu_3|\le \aleph_0.
$$
In addition, every probability measure $\mu$ is a regular Borel measure, thus we can use the above decomposition for any $\mu$ of interest. To see this, notice that $\mu$ is automatically Borel by definition, and therefore regular because any Borel probability measure on a compact metric space (including $[0,1]$) is known to be regular.

\textbf{EAS-learnable:}
By the tight characterization of EAS-learnability \cite{wu2021non}, for any $\mu$, $\mathcal{H}$ is EAS-learnable if and only if there is a countable subset $\mathcal{H}'$ of $\mathcal{H}$, such that for any $h\in \mathcal{H}$, there exists $h'\in \mathcal{H}'$ satisfying
$$
\mu(\{x| h(x)\ne h'(x)\})=0.
$$
In this case, we consider $\mathcal{H}'$ to be the union of two sets
$$
\mathcal{H}'=\{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|<\infty, a_i,b_i\in \mathbb{Q}\}\cup \{h:|h^{-1}(1)|<\infty, h^{-1}(1)\subset \textbf{supp}(\mu_3)\}.
$$
Because a countable union of countable sets is still countable, the two sets above are both countable. In particular, for the first set we denote 
$$\mathcal{H}_n=\{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|=n, a_i,b_i\in \mathbb{Q}\},$$
then each $\mathcal{H}_n$ is countable and 
$$\{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|<\infty, a_i,b_i\in \mathbb{Q}\}=\cup_{n\in \mathbb{N}^+}\mathcal{H}_n.$$
For the second set, notice there is a natural bijective mapping between it and $\mathbb{N}$ in the binary numeral system.

Now we show that for any $h\in \mathcal{H}$, there exists $h'\in \mathcal{H}'$ satisfying
$$
\mu(\{x| h(x)\ne h'(x)\})=0.
$$
Since any $h\in \{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|<\infty, a_i,b_i\in \mathbb{Q}\}$ is in $\mathcal{H}'$, we only need to consider $h\in \{h:|h^{-1}(1)|<\infty\}$. We pick $h'$ such that $h^{-1}(1)=h^{' -1}(1)$ on $\textbf{supp}(\mu_3)$. Because $\mu_1,\mu_2$ are continuous, we have that
$$
(\mu_1+\mu_2)(h^{-1}(1))=(\mu_1+\mu_2)(h^{' -1}(1))=0.
$$
By the choice of $h'$, it coincides with $h$ on $\textbf{supp}(\mu_3)$, thus $\mu_3(\{x| h(x)\ne h'(x)\})=0$.

\textbf{Not Strongly-EAS-learnable:}
We first restrict our attention to only deterministic algorithms, which was considered in \cite{wu2021non}. The high-level idea is that when $\mu$ is unknown, a deterministic algorithm can never exclude either $\{h:|h^{-1}(1)|<\infty\}$ or $\{h: h^{-1}(1)=\cup_{i\in I} [a_i,b_i], |I|<\infty, a_i,b_i\in \mathbb{Q}\}$. We will show for any deterministic algorithm, there exists a $\mu, h$ pair that it makes infinite mistakes on.

Consider a discrete probability measure with $\textbf{supp}(\mu)=\cup_{i\in \mathbb{N}^+} x_i$. Denote $t(i)$ to be the first time that the learner encounters the $ith$ new point $y_i\in \textbf{supp}(\mu)$. If the algorithm predicts 0 at time $t(i)$, it makes a mistake on any $h$ of the second kind which includes $[a_j,b_j]$ that contains $y_i$. If the algorithm predicts 1 at time $t(i)$, it makes a mistake on any $h$ of the first kind where $y_i\in h^{-1}(1)$. 

We count the number of 1's the learner predicts. 

(why it works on known distribution?)

something like diagonal deletion?

construct an uncountable set, where each element is a countable set, such that the restriction to any countable set is countable.

bad examples: (1) fixed countable + one changing real number (2) uncountable disjoint sets

countable cover with finite error?

\end{proof}

\begin{definition}[Strategy of Nature]
    A (deterministic) strategy $S$ of Nature, is any function from $A$ to $\mathcal{X}^{\aleph_0}$, where $A$ denotes the set of all algorithms, and $\mathcal{X}^{\aleph_0}$ denotes the set of all countable ordered sequences with each element being an element from $\mathcal{X}$.
\end{definition}

There are a few settings $x_t$ and $h_t^*$ are chosen by Nature, corresponding to different levels of adaptivity. We list below the settings from the weakest to the strongest, where a setting is said to be learnable if there exists an algorithm which makes finite errors with probability 1 for the first two settings, and is said to be learnable if there exists an algorithm which makes finite errors for the latter four settings.

\begin{definition}[EAS Learnable]
    A fixed arbitrary probability measure $\mu$ is revealed to both parties in advance. $x_t$ are iid samples from $\mu$. $h_t^*\equiv h^*$ is fixed by Nature in advance.
\end{definition}

\begin{definition}[Strongly-EAS Learnable]
    An arbitrary probability measure $\mu$ is fixed by Nature in advance. $x_t$ are iid samples from $\mu$. $h_t^*\equiv h^*$ is fixed by Nature in advance.
\end{definition}

\begin{definition}[Adaptive-EAS Learnable]
    $x_t$ is chosen by Nature with an arbitrary $S$. $h_t^*\equiv h^*$ is fixed by Nature in advance.
\end{definition}

\begin{definition}[Pointwise-Adaptive-EAS Learnable]
    $x_t$ is chosen by Nature with an arbitrary $S$. $h_t^*\equiv h^*$ is fixed by Nature in advance. In addition, for any $h^*$, we require a uniform upper bound on the number of errors made.
\end{definition}

\begin{definition}[Uniform-Adaptive-EAS Learnable]
    $x_t$ is chosen by Nature with an arbitrary $S$. $h_t^*\equiv h^*$ is fixed by Nature in advance. In addition, we require a uniform upper bound on the number of errors made.
\end{definition}

\begin{definition}[Online Learnable]
    $x_t$ is chosen by Nature with an arbitrary $S$. $h_t^*$ is chosen by Nature under the restriction that $h_t^*(x_i)=h_i^*(x_i), \forall i<t$.
\end{definition}

It's clear there is an inclusion relation between the settings above:
$$
\text{Online} \subset \text{UAEAS} \subset \text{PAEAS} \subset \text{AEAS} \subset \text{SEAS} \subset \text{EAS}.
$$
In addition, online learnability is known to be equivalent to $\mathcal{H}$ having a finite Littlestone dimension \cite{littlestone1988learning}, and EAS learnability is known to be equivalent to $\mathcal{H}$ being effectively countable w.r.t $\mu$ \cite{wu2021non}. Within the scope of this work, we will only consider deterministic algorithms for the learner, since the tight guarantees for both online and EAS learnabilities are achieved by deterministic algorithms as well.

We have two main aims: (1) to characterize pointwise-adaptive-EAS learnability, uniform-adaptive-EAS learnability, adaptive-EAS learnability and strongly-EAS learnability, (2) to decide whether the inclusion relations are strict. Notice that solving (2) will directly answer an open question of \cite{wu2021non}.

Consider countable union of little stone. exponentially weighted average forecaster for countable experts, 0/1 loss? the bayes algorithm

when it's countable union of little stone, it's tight in terms of T, and there is no appropriate criteria on other dependences since it's non-uniform

problem, agnostic needs to know T. need an infinite horizon version for agnostic with finite littlestone

countable sub experts, can use bayes twice! might not be pointwise! cluster by the end time (log poly t)

PFL, remark can do better but not necessary

computationally inpractical

can we prove whenever it's not countable union of little stone, it breaks? an example is easy

\begin{example}
    Consider $\mathcal{X}=[0,1]$, and the class of all finite-support functions
$$
\mathcal{H}=\{h: |h^{-1}(1)|<\infty\}.
$$
This hypothesis class has infinite Littlestone dimension, thereby not uniform online learnable. However, We have the countable decomposition $\mathcal{H}=\cup_{n\in \mathbb{N}^+} \mathcal{H}_n$, where
$$
\mathcal{H}_n= \{h: |h^{-1}(1)|\le n\}.
$$
It's easy to verify each $\mathcal{H}_n$ has finite Littlestone dimension $n$.
\end{example}

\iffalse
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
    \caption{Expert$(i_1,\cdots,i_L)$}
    \label{expert}
    \begin{algorithmic}[1]
        \STATE Input: a hypothesis class $\mathcal{H}$, indices $i_1<\cdots<i_L$.
        \STATE Initialize the active hypothesis set $V_1=\mathcal{H}$.
        \FOR{$t\in \mathbb{N}^+$}
        \STATE Observe $x_t$.
        \STATE For $y\in \{0,1\}$, let $V_t^{y}=\{h: h(x_t)=y, h\in V_t\}$.
        \STATE Predict $\hat{y}_t=\text{argmax}_y \textbf{Ldim}(V_t^{y})$.
        \STATE Observe the true label $y_t$.
        \STATE Update $V_{t+1}=V_t^{y_t}$ if $y_t\ne \hat{y}_t$ and $t\in \{i_1,\cdots,i_L\}$. Otherwise set $V_{t+1}=V_t$.
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
    \caption{Follow the Perturber Leader (FPL)}
    \label{fpl}
    \begin{algorithmic}[1]
        \STATE Input: a countable class of experts $E_1,E_2,\cdots$. 
        \STATE Initialize a complexity $k_i$ for each expert $E_i$, such that $\sum_{i\in \mathbb{N}^+} e^{-k_i}\le 1$.
        \FOR{$t\in \mathbb{N}^+$}
        \STATE Choose learning rate $\eta_t$.
        \STATE Sample a random vector $q\sim \text{exp}$, i.e. $\mathbb{P}(q_i=\lambda)=e^{-\lambda}$ for $\lambda \ge 0$ and all $i\in \mathbb{N}^+$.
        \STATE Output prediction $\hat{y}_t$ of expert $E_i$ which minimizes
$$
\sum_{j=1}^{t-1}1_{[E_i(x_j)\ne y_j]}+\frac{k_i-q_i}{\eta_t}.
$$
        \STATE Observe the true label $y_t$.
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\fi

Lemma \ref{online} characterizes a worst-case uniform finite error bound on $\mathcal{H}$. However, there exists examples with arbitrary-depth shatter trees but without an infinite-depth shatter tree, which sometimes admit a non-uniform finite error bound.

\begin{example}\label{ex1}
    Consider $\mathcal{X}=\mathbb{N}^+$ and let $\mathcal{H}$ be the set of all threshold functions
    $$
    \mathcal{H}=\{h: h(x)=1_{[x\ge n]}, n\in \mathbb{N}\}.
    $$
    The Littlestone dimension $\textbf{Ldim}(\mathcal{H})=\infty$. However, there is a simple learning algorithm guaranteeing finite error, by keeping predicting 0 until the first mistake, which means the set of consistent hypotheses is finite. 
\end{example}

We notice that this example differs from example \ref{ex1} in that it's doesn't even have a non-uniform finite error bound in the online setting, showing that fixing $h^*$ does distinguish our setting from the classic online learning setting. To see this, notice that the infinite sequence $(\frac{1}{2},\frac{1}{4},\frac{3}{4},\frac{1}{8},\cdots)$ forms a shatter tree with infinite depth.

\subsection{EAS}

we strengthen a result of EAS, its indeed non-uniform!

when the sigma-algebra is separable

\zl{to do, relation to strong eas in simple setting, or at least eas?}

\zl{equal to strong eas true for countable domain.}

if we want to prove separation

consider uncountable number of countable set, each other are same/different on countable set, (each 1 point is 0/1 on infinity hypotheses). this is a necessary condition of not non-uniform. if we can should it plus eas implies not non-uniform, it means it's a n/s condition of not non-uniform.

Can we further strengthen such condition to be not non-uniform?

can we construct eas, such that any uncountable subset is not LS? need to construct the worst eas

\zl{try this}

Consider the function class $\mathcal{F}$ on $[0,1]$. For any real number $c\in (0,1)$, we define a set $S_c$:
$$
S_c=\{c,\frac{1+c}{2},\frac{3+c}{4},\cdots\},
$$
and accordingly a hypothesis
$$
f_c(x)=1_{x\in S_c}.
$$
Clearly $\mathcal{F}$ is EAS. We try to show for any countable partition of $\mathcal{F}$, there is one of them (which is uncountable), such that it "simulates" a threshold which is not a Littlestone class.

\zl{problem, they can be disjoint}

\begin{example}
    Consider $\mathcal{X}=[0,1]$, and the class of all finite-support functions
$$
\mathcal{H}=\{h: |h^{-1}(1)|<\infty\}.
$$
This hypothesis class has infinite Littlestone dimension, thereby not uniform online learnable. However, We have the countable decomposition $\mathcal{H}=\cup_{n\in \mathbb{N}^+} \mathcal{H}_n$, where
$$
\mathcal{H}_n= \{h: |h^{-1}(1)|\le n\}.
$$
It's easy to verify each $\mathcal{H}_n$ has finite Littlestone dimension $n$.
\end{example}

We begin with a brief description of a Gale-Stewart game and how we relate it to consistency, borrowed from \cite{bousquet2021theory} (readers familiar with it can skip this part).

Consider the non-uniform online learning game from a different perspective: for $x_1,\cdots,x_t\in \mathcal{x}$ and $y_1,\cdots,y_t\in \{0,1\}$, consider the class
$$
\mathcal{H}_{x_1,y_1,\cdots,x_t,y_t}=\{h\in \mathcal{H}: h(x_i)=y_i, \forall 1\le i\le t\}.
$$
of consistent hypotheses. Nature tries to maximize the number of errors Learner makes by choosing a sequence with $y_t\ne \hat{y}_t$ for as many initial rounds in a row as possible. In other words, Nature tries to keep 
$$
\mathcal{H}_{x_1,1-\hat{y}_1,\cdots,x_t,1-\hat{y}_t}\ne \emptyset
$$
as long as possible. When this set becomes empty, the only
consistent choice of label is $y_t=\hat{y}_t$, so Learner makes no errors from now on.

Define the following game $\mathcal{G}$, with two players $P_L$ and $P_N$. At each round $t$, $P_N$ chooses a point $x_t\in \mathcal{X}$ and shows it to $P_L$, then $P_L$ chooses a point $z_t\in\{0,1\}$.

$P_L$ wins the game in round $t$ if $\mathcal{H}_{x_1,z_1,\cdots,x_t,z_t}=\emptyset$. $P_N$ wins the game if the game continues indefinitely. In other words, the set of winning sequences for $P_L$ is 
$$
W=\{(x,z)\in (\mathcal{X}\times \{0,1\})^{\infty}: \mathcal{H}_{x_1,z_1,\cdots,x_t,z_t}=\emptyset\ \text{for some}\ t<\infty\}.
$$
This set of sequences $W$ is finitely decidable because the membership of $(x,z)$ in $W$ is witnessed by a finite subsequence. Thus the above game is a Gale-Stewart game. By the Borel determinacy theorem, exactly one of $P_L$ or $P_N$ has a winning strategy. We have the following lemma relating this game to the definition of a realizable infinite-depth shatter tree.

\begin{lemma}
    $P_N$ has a winning strategy in $\mathcal{G}$, if and only if $\mathcal{H}$ has a realizable infinite-depth shatter tree.
\end{lemma}
\begin{proof}\textbf{If:} suppose $\mathcal{H}$ has a realizable infinite-depth shatter tree. For each branch $x$ of the tree we choose one of its corresponding consistent hypothesis $h_x$, then for each $x$ we create a $P_N$ strategy $S_x$ which simply feeds $x_t$ to $P_L$ at time $t$. Since $P_L$ is deterministic, 

\textbf{Only if:}
    
\end{proof}

Now we are ready to prove the theorem.

As a preliminary study on the new direction of explaining inductive inference via online learning, our result has some limitations and potential opportunities for future research as well. The characterization of learnability in the agnostic setting is less complete than our results in the realizable setting, we wonder if there is a dichotomy that an $o(T)$ regret is impossible whenever $\mathcal{H}$ can't be written as a countable union of Littlestone classes. 

In addition, this work assumes a bias in the hypothesis class ($\mathcal{H}$ as a subset of $\mathcal{S}$), while it remains unclear what's a good choice $\mathcal{H}$, or how to model the process of generating $\mathcal{H}$. It's widely believed there is some intrinsic bias in the law of Nature, for example the Occam's razor, which accounts for success of learning. However, it's also likely that the bias itself, no matter what it is, leads to such success of learning, and people choose the bias towards simplicity because it's cheap.

\zl{a good class is falsible?}

\zl{non-uniform vs consistent}

\subsection{Proof of Proposition \ref{thm con}}
\begin{proof}
    Suppose $\mathcal{H}$ has a realizable infinite-depth shatter tree. For each branch $x$ we choose one of its corresponding consistent hypothesis $h_x$, then for each $h_x$ we create a Nature's strategy $S_x$ which simply fixes $h_x$ and feeds $x_t$ to Learner. Since Learner is deterministic, when the way Nature generates $x$ is under the restriction of the tree, denote $\hat{y}$ as the prediction of Learner when it makes an error every round. There is a unique branch $x$ determined by $y=1-\hat{y}$ on the tree. Then $S_x$ satisfies $\hat{y}_t\ne y_t, \forall t$ is the desired strategy of Nature. \zl{to make precise}
\end{proof}

\iffalse
Theorem \ref{thm ag} asserts that for any sequence of $x,y$ and horizon $T$, the regret w.r.t. the best hypothesis $h^*$ in hindsight is $O(\sqrt{T})$ if the hypothesis class can be written as a countable union of Littlestone classes. A natural question is whether it's a tight characterization of all agnostic non-uniform learnable classes. We show that for the slightly stronger (but also conventional) criteria requiring $O(\sqrt{T})$ regret w.r.t. $h^*$ for any sequence of $x,y$ and horizon $T$ (here $h^*$ will depend on $x,y,T$), any class $\mathcal{H}$ that's not a countable union of Littlestone classes can't have sub-linear regret.

\begin{proposition}\label{ag con}
     Define $h^*=\text{argmin}_{h\in \mathcal{H}}\sum_{t=1}^T 1_{[h(x_t)\ne y_t]}$ as a function of $x,y,T$. If a hypothesis class $\mathcal{H}$ is not a countable union of Littlestone classes, then for any $\epsilon>0$, there doesn't exist function m: $\mathcal{H}\to \mathbb{N}^+$, such that $\forall x\in X, \forall y\in \{0,1\}^{\infty}, \forall T\in \mathbb{N}^+$,
     $$
\mathbb{E}\left[\sum_{t=1}^T 1_{[\hat{y}_t\ne y_t]}-
\sum_{t=1}^T 1_{[h^*(x_t)\ne y_t]}\right]\le m(h^*) T^{1-\epsilon}.
$$
\end{proposition}
\zl{tbd}
\fi

As for the stochastic setting where $x_t$ is drawn independently from an unknown fixed probability measure, the same regret upper bound holds. On the other hand, it's well known an $\Omega(\sqrt{T})$ lower bound is inevitable.

\begin{proposition}\label{prop}
    Consider the simple problem where $\mathcal{X}=\{0\}$ and $\mathcal{H}=\{h_0(0)= 0, h_1(0)= 1\}$. There is a choice of Nature generating $y_t$, such that for any algorithm and and $T\in \mathbb{N}^+$, the expected regret at time $T$ is $\Omega(\sqrt{T})$. 
\end{proposition}

As a result, the regret bound of Theorem \ref{thm ag} is tight in terms of the dependence on $T$ in the stochastic setting, which can be seen as an accumulated regret analogue to the per-iteration generalization result of \cite{bousquet2021theory} in the agnostic setting, which they left as a future direction. 

\iffalse
We also show that, similar to Theorem \ref{thm con}, having no $\aleph_1$-size tree is a necessary condition for sub-linear rate in the agnostic setting. 

\begin{theorem}\label{ag con}
    If a hypothesis class $\mathcal{H}$ is agnostic non-uniform learnable at rate $O(T^{1-\epsilon})$ for some constant $\epsilon>0$, then it doesn't have any $\aleph_1$-size tree in which tree nodes belong to $\mathcal{X}$.
\end{theorem}
\fi

==> check.tex <==
\section*{NeurIPS Paper Checklist}


 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we make sure all the claims are accurate.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we discuss the limitations and future directions for improvement in the Discussion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we provide the full set of assumptions for all theoretical results. We provide a complete (and correct) proof to for all theoretical results, among which the simpler ones are left to the appendix.
    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: paper does not include experiments requiring code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we carefully follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: there is no societal impact of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not use existing assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> conjecture.tex <==
\section{Conjecture on Factorizing Littlestone Classes}

For any set $S$ which contains disjoint subsets of $\mathcal{X}$, and a base hypothesis $h^*$, we define the following hypothesis class which we will call a basic class $n$-generated by $(h^*,S)$ (the set $\cup_{i=1}^n s_i$ is set $\emptyset$ when $n=0$).
$$
\mathcal{H}_{n}(h^*,S)=\{h\in \mathcal{S}: \{h\ne h^*\}= \cup_{i=1}^n s_i, s_i\in S, n\in \mathbb{N}\}.
$$
We pose the following conjecture on the canonical factorization of Littlestone classes.

\begin{conjecture}[Canonical Factorization of Littlestone Classes]\label{decom}
    A hypothesis class $\mathcal{H}$ has finite Littlestone dimension, if and only if it's a subset of a finite union of basic classes:
    $$
    \mathcal{H}\subset \cup_{j=1}^m \mathcal{H}_{n_j}(h_j^*,S_j), \text{where}\ n_j, m\in \mathbb{N}^+.
    $$
\end{conjecture}

This conjecture, if proven, will not only simplify the characterization of non-uniform online learnability, but also imply a more practical algorithm for classic online learning. For non-uniform online learnability, it would be equivalent to saying $\mathcal{H}$ is a countable union of basic classes.

For classic online learning, the crucial issue limiting the practical use of SOA is its intractability: SOA requires computing the Littlestone dimension of two new hypothesis classes each round, while there is no efficient method for such computation. If the conjecture is true, we only need to compute the canonical factorization of $\mathcal{H}$ once in advance, then there is a trivial algorithm that online learns $\mathcal{H}$: starting with $j=1$, Learner plays according to $h_j^*$ and remembers the errors until $n_j+1$ errors are made, then goes to $j+1$ and repeat the procedure.

We only proved the case $\textbf{Ldim}(\mathcal{H})=1$ for the conjecture.

\begin{proof}
    The if direction is straightforward: Learner can simply run SOA on $\mathcal{H}_{n_1}(h_1^*,S_1)$ which clearly has Littlestone dimension $n_1$, then switch to $\mathcal{H}_{n_2}(h_2^*,S_2)$ until he made $n_1+1$ mistakes. Learner repeats this process for $j=1,\cdots,m$, and makes at most $m+\sum_{j=1}^m n_j$ mistakes.

    For the only if direction, we first consider the case $\textbf{Ldim}(\mathcal{H})=1$. Without loss of generality we assume $h_0: h_0(x)\equiv 0, \forall x\in \mathcal{X}$ is in $\mathcal{H}$. Now, for any point $x$ such that there exists some $h_x\in \mathcal{H}, h_x(x)=1$, by the definition of Littlestone dimension, we have that one of the following is a singleton:
    $$
    H_x(0)=\{h\in \mathcal{H}: h(x)=0\}, H_x(1)=\{h\in \mathcal{H}: h(x)=1\}.
    $$
    If $H_x(0)$ is a singleton, then for any $h\in \mathcal{H}, h\ne h_0$, we have that $h(x)=1$. If $H_x(1)$ is a singleton, then $|\{h\in \mathcal{H}: h(x)=1\}|=1$. Denote $X^*$ as the set of points $x$ that all $h\in \mathcal{H}$ but $h_0$ satisfies $h(x)=1$. For any $h\in \mathcal{H}, h\ne h_0$, denote $X_h=\{x\in \mathcal{X}: h(x)=1, x\notin X^*\}$. We have that $X_{h_1} \cap X_{h_2}=\emptyset, \forall h_1,h_2 \in \mathcal{H} \setminus h_0$ by the property of singleton $H_x(1)$. Define $h^*: h^*(x)=1\ \textbf{iff}\ x\in X^*$, we have the following desired decomposition:
    $$
    \mathcal{H}\subset \mathcal{H}_{1}(h^*,\cup_{h\in \mathcal{H} \setminus h_0} \{X_h\}) \cup \mathcal{H}_{0}(h_0,\emptyset)= \mathcal{H}_{1}(h^*,(\cup_{h\in \mathcal{H} \setminus h_0} \{X_h\})\cup \{X^*\}).
    $$
    It's easy to verify the inclusion $\mathcal{H}\subset \mathcal{H}_{1}(h^*,(\cup_{h\in \mathcal{H} \setminus h_0} \{X_h\})\cup \{X^*\})$ also holds for general $h^*$ without the restriction about the choice of $h_0$.
    
\end{proof}

==> rebuttal.tex <==
\section{Rebuttal}

\subsection{Reviewer 1}
Thank you for your valuable feedback! We will address your concerns here.

More explanation on equivalence: the equivalence is discussed in lines 140-147. Since our framework is a strictly more general form than previously considered inductive inference by removing constraints on $\mathcal{H}$ and $x_t$, we believe it's redundant to have side-by-side mathematical definitions again (as opposed to line 67). We give a representative example of how the problem of learning computable functions is subsumed by our framework in lines 143-147. 

Different rules of observations: it refers to different Nature's choices of observations $x_t$. Here Definition 4 formulates the adversarial case while Definition 5 handles the stochastic case. By Theorem 9 and Theorem 11, we prove that the two cases share the same sufficient and necessary condition, which implies this condition is also sufficient and necessary for any "rule of observation" between the adversarial and stochastic cases. This corresponds to "different rules of observations" in line 141. 

If our explanation on the equivalence still feels unclear to you, please provide further suggestions and we will improve our writing correspondingly.

More examples: we put the examples in the appendix due to space limit, we will add some key examples back to the main paper for readability as you suggested. Below we answer your questions.

A countable union of Littlestone classes but not countable: we give a stronger example which is a Littlestone class with an uncountable size. Consider the set of indicator functions on $[0,1]$, i.e. $\{f_c| f_c(x)=1_{x=c}, c\in [0,1]\}$. The size of this hypothesis class is uncountable because $[0,1]$ has the same cardinality as $\mathbb{R}$. This class itself has Littlestone dimension 1. A naive algorithm that makes at most one error on this class is the following: always predict $y_t=0$ until making the first error on some $x_t=c$, then the ground-truth $h^*$ is identified as $f_c$ and we predict w.r.t. $f_c$ afterwards.

Not non-uniform learnable but consistent: this is left as an open question, as shown in Table 1. Currently we only know non-uniform learnablity is a subset of consistency and we obtained a new necessary condition for consistency (Theorem 18). It's unclear whether consistency can be separated from non-uniform learnablity or not.

If our response has addressed your concerns, please consider reevaluate our paper. If you have further questions, please let us know. Thank you again for your valuable time and insights!

\subsection{Reviewer 2}
Thank you for your valuable feedback! We will address your concerns here.

Practical implications: this work is devoted to a conceptual link between philosophy and learning theory, therefore practical implication is not the primary objective and is beyond the scope of the current work. Still, our algorithm has the potential to be made more practical by designing approximate algorithms (as we briefly mentioned in future directions). The original form of Solomonoff induction is also known to be intractbale, but later works built approximate versions of Solomonoff induction. Some recent works are studying the practical use of inductive inference in large language models (for example, "Learning Universal Predictors" by Grau-Moya et al 2024), and we believe our algorithms have the potential to be useful in practice similarly, for understanding if large language models implicitly learn such Bayesian algorithms during inference.

\subsection{Reviewer 3}
Thank you for your valuable feedback! We will address your concerns here.

Connection to computational complexity (page 1): good point! Inductive inference (especially Solomonoff's method) is not only linked to learning theory but also to the theory of computation. We will add some discussion on this connection (we find the paper "Learning in Pessiland via Inductive Inference" by the authors you mentioned indeed has implications to machine learning).

Comparison between pseudocodes (page 2): we list them side by side for a straightforward comparison. Only lines 2,6,9 are different. Here lines 2,6 correspond to the difference in protocols: classic online learning allows a changing ground-truth (line 6), while inductive inference requires the ground-truth to be fixed in advance (line 2). Line 9 corresponds to the difference in criteria: classic online learning requires uniform error bounds, while inductive inference allows the bounds to depend on the ground-truth. We will add a caption to briefly explain the differences.

Lines 140-147 (page 4): this paragraph conveys two messages (1) our framework considers general $\mathcal{H}$, while previous work on inductive inference only considers $\mathcal{H}$ with a countable size (2) our framework incorporates different setting on how Nature chooses $x_t$ (adversarial or stochastic), while most previous work only considers a certain rule of nature's choice on $x_t$. By these two, we reach the conclusion that our framework is a general framework of inductive inference, subsuming the previously considered settings. As an example, we cast the problem of  learning computable functions under our framework. If this makes more sense to you, we will rewrite this paragraph to make it more clear.

Lines 179-181 (page 5): once $A_n$ makes more than $d_k+k$ errors at some time step $t_0$, then for any $t> t_0$, $e(t,n)\ge d_k+k$, and $e(t,n)+n> d_k+k$ since $n\ge 1$. By the definition of how we pick the index $J_t$ (line 5 in Algorithm 1), index $k$ will always be strictly better than index $n$ for any $t> t_0$ because $e(t,k)+k\le  d_k+k$, then our algorithm will never pick $J_t=n$ after $t_0$. Combining it with the fact that only indexes no larger than $d_k+k$ can be possibly invoked, we make at most $(d_k+k)^2$ errors.

Choice of $x^{n(h)+1}$ (page 6): $n(h)+1$ is the smallest number $n$ that guarantees a contradiction, for which we want $n>n(h)$.

Notion of regret (page 7): the regret notion in Theorem 12 is from Definition 6. It's a natural extension of the regret notion in agnostic online learning to the non-uniform setting: we require a uniform dependence on $T$ ($r(T)$ is the same across different $h$), while the overhead $m(h)$ can vary with different $h$.

Lines 268-269 (page 8): Figure 1 can serve as an intuitive explanation. Roughly speaking, we use the claim from lines 261-262 multiple times, to find a sub-tree which is a binary tree with depth $m^*+2$, each node being the root of an $\aleph_1$-size tree. In Figure 1, $v_{(1,1)}$ is the ancestor of the sub-tree, with $v_{(2,1)}$ and $v_{(2,2)}$ being its children (though $v_{(2,1)}$ is not its child in the original tree).

Future work (page 9): as we briefly mentioned, our learning algorithms are inevitably intractable, and we leave a computationally tractable approximate algorithm for future work.

==> vsproof.tex <==
\section{Proof of Theorem \ref{thm con}}
We begin with a brief description of a Gale-Stewart game and how we relate it to consistency, borrowed from \cite{bousquet2021theory} (readers familiar with it can skip this part).

Consider the non-uniform online learning game from a different perspective: for $x_1,\cdots,x_t\in \mathcal{x}$ and $y_1,\cdots,y_t\in \{0,1\}$, consider the class
$$
\mathcal{H}_{x_1,y_1,\cdots,x_t,y_t}=\{h\in \mathcal{H}: h(x_i)=y_i, \forall 1\le i\le t\}.
$$
of hypotheses consistent with the observed sequence. Nature who tries to maximize the number of errors the learner makes will choose a sequence with $y_t\ne \hat{y}_t$ for as many initial rounds in a row as possible. In other words, Nature tries to keep 
$$
\mathcal{H}_{x_1,1-\hat{y}_1,\cdots,x_t,1-\hat{y}_t}\ne \emptyset
$$
as long as possible. When this set would become empty, the only
consistent choice of label is $y_t=\hat{y}_t$, so the learner makes no errors from that point onwards.

We define the following game $\mathcal{G}$, with two players $P_L$ and $P_N$. At each round $t$, $P_N$ chooses a point $x_t\in \mathcal{X}$ and shows it to $P_L$, then $P_L$ chooses a point $z_t\in\{0,1\}$.

$P_L$ wins the game in round $t$ if $\mathcal{H}_{x_1,z_1,\cdots,x_t,z_t}=\emptyset$. $P_N$ wins the game if the game continues indefinitely. In other words, the set of winning sequences for $P_L$ is 
$$
W=\{(x,z)\in (\mathcal{X}\times \{0,1\})^{\infty}: \mathcal{H}_{x_1,z_1,\cdots,x_t,z_t}=\emptyset\ \text{for some}\ t<\infty\}.
$$
This set of sequences $W$ is finitely decidable in the sense that the membership of $(x,z)$ in $W$ is witnessed by a finite subsequence.


\begin{proof}
    \textbf{Only if:} suppose $\mathcal{H}$ has a realizable infinite-depth shatter tree. For each branch $x$ we choose one of its corresponding consistent hypothesis $h_x$, then for each $h_x$ we create a Nature's strategy $S_x$ which simply fixes $h_x$ beforehand and choose $x_t$ according to the shatter tree.

    \textbf{If:}
\end{proof}
